APX-Hardness of the Minimum Vision Points Problem

Placing a minimum number of guards on a given watchman route in a polygonal domain is called the {\em minimum vision points problem}. We prove that finding the minimum number of vision points on a shortest watchman route in a simple polygon is APX-Hard. We then extend the proof to the class of rectilinear polygons having at most three dent orientations.

==> Figures/intersect <==
#!/usr/bin/python
#
# 'intersection' takes two line segments (eight coordinates) and computes the intersection point of the segments. 
# 

import sys


def minus(v1,v2): return [v1[0]-v2[0],v1[1]-v2[1]]

def intersection(p1,q1,p2,q2):
    # Find s,t s.t. (1-s)*p1+s*q1 = (1-t)*p2+t*q2
    print p1, q1, p2, q2
    u1 = minus(q1,p1)
    u2 = minus(q2,p2)
    v  = minus(p2,p1)
    print u1, u2, v,
    t  = (v[1]*u1[0]*1.0-v[0]*u1[1]*1.0)/(u2[0]*u1[1]*1.0-u2[1]*u1[0]*1.0)
    print t
    return [p2[0]+t*u2[0],p2[1]+t*u2[1]]

lines = [[[0,0],[0,0]],[[0,0],[0,0]]]
arg = 1
try:
    for segment in range(2):
        for point in range(2):
            for coord in range(2):
                lines[segment][point][coord] = int(sys.argv[arg])
                arg +=1
except: 
    print "Provide two line segments, eight integer coordinates in the format 'x11 y11 x12 y12 x21 y21 x22 y22'!\nExiting program!!!"
    sys.exit(0)

print lines
print "Intersection point is:\n"+str(intersection(lines[0][0],lines[0][1],lines[1][0],lines[1][1]))



==> Figures/reflect <==
#!/usr/bin/python
#
# 'reflect' takes a line segment (four coordinates) and at least one point (two coordinates each) 
#  and computes the reflection of each point along the line. 
# 

import sys


def dot(v1,v2): return v1[0]*v2[0]*1.0 + v1[1]*v2[1]*1.0

def minus(v1,v2): return [v1[0]-v2[0],v1[1]-v2[1]]

def reflect(point,segment): 
    u = minus(segment[1],segment[0])
    v = minus(point,segment[0])
    q = [segment[0][0] + u[0]*dot(u,v)/dot(u,u), segment[0][1] + u[1]*dot(u,v)/dot(u,u)]
    print "middle="+str(q)
    return minus([2.0*q[0],2.0*q[1]],point)

line  = [[0,0],[0,0]]
point = [0,0]
try:
    arg   = 1
    for p in range(2):
        for coord in range(2):
            line[p][coord] = int(sys.argv[arg])
            arg += 1
    s = ''
    for i in range(5, len(sys.argv), 2):
        point[0] = int(sys.argv[i])
        point[1] = int(sys.argv[i+1])
        s       += "\n"+str(point)+" reflects to: "+str(reflect(point,line))
except: 
    print "Provide a line segment and at least one point, at least six integer coordinates in the format 'x11 y11 x12 y12 x y x y...'!\nExiting program!!!"
    sys.exit(0)

print line, s


